Exploring the Impact of Human Evaluator Group on Chat-Oriented Dialogue Evaluation

Human evaluation has been widely accepted as the standard for evaluating chat-oriented dialogue systems. However, there is a significant variation in previous work regarding who gets recruited as evaluators. Evaluator groups such as domain experts, university students, and professional annotators have been used to assess and compare dialogue systems, although it is unclear to what extent the choice of an evaluator group can affect results. This paper analyzes the evaluator group impact on dialogue system evaluation by testing 4 state-of-the-art dialogue systems using 4 distinct evaluator groups. Our analysis reveals a robustness towards evaluator groups for Likert evaluations that is not seen for Pairwise, with only minor differences observed when changing evaluator groups. Furthermore, two notable limitations to this robustness are observed, which reveal discrepancies between evaluators with different levels of chatbot expertise and indicate that evaluator objectivity is beneficial for certain dialogue metrics.

==> tex/ethics.tex <==
\section{Ethics Statement}

This work presents findings that are useful for improving the quality of human evaluation of chat-oriented dialogue models. In particular, we explore the effect that changing evaluator group has on dialogue evaluation results. Our analyses will allow researchers to make more informed decisions and interpretations of dialogue model evaluations.

This work relies on the evaluation of real human-bot conversations; however, we do not collect new dialogue data and instead leverage an anonymized, publicly available dialogue dataset from the \citet{finch:23} study. \citet{finch:23} screened this data for any personally identifiable information in their work.

When evaluating human-bot conversations, there is also a small risk of conversations containing triggering or offensive content to the evaluator from either the utterances of the human interactor or of the dialogue model. \citet{finch:23} explicitly instructed the human interactors to refrain from such antisocial behavior and also reported dramatically low rates of antisocial bot utterances (near 0\% for all conversations). As a result, the utilized dataset does not carry this risk. 

The human evaluators used in this work were USA-based and paid at a rate above the federal USA minimum wage of \$10/hour for $Stu_x$ and $Dev_x$. The per-task payment rate was based on the results of pilot studies which afforded time estimates for the completion of the different evaluation tasks. Participation by human evaluators was entirely voluntary. Evaluators were able to opt-out of the study at any time. Evaluators were given a clear description of their responsibilities and the compensation structure before being given any work. These measures ensure that the participation of our human evaluators was fair, transparent, and benefited their interests.

==> tex/fig/agreements.tex <==

\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{tex/img/agreements_with_significance.pdf}
\caption{IAA (Krippendorf's alpha) for between-group and within-group evaluations: $Stu$-vs-$Sur$ raters (red) and $Sur$-vs-$Sur$ raters (gray). Error bars denote 95\% confidence intervals from bootstrapping.}
\label{fig:agreements}
\end{figure*}

% \begin{figure*}[htb]
% \centering
% \includegraphics[width=\textwidth]{tex/img/agreement_proportions_with_significance.pdf}
% \caption{Proportions of flat agreement between different rater groups: interactive-vs-external raters (red) and external-vs-external raters (gray). Boxed labels indicate statistically significant differences between the two rater groups (z-test of proportions, \textit{p} < 0.05).}
% \label{fig:agreement_proportions}
% \end{figure*}

==> tex/fig/comparative_ranking.tex <==

\begin{figure}[htb]
\centering
\includegraphics[width=\columnwidth]{tex/img/comparative_ranking_uisx.png}
\caption{The proportion of bootstrapped samples (n=1000) of conversation-pairs (100 per bot) for which the bot rankings are the same. Bars denote ranking agreement for between-group $Stu$-$Sur$. Lines denote ranking agreement for within-group $Stu$ and $Sur$.}
\label{fig:comparative_ranking}
\end{figure}

==> tex/fig/likert_ranking.tex <==

\begin{figure}[htb]
\centering
\includegraphics[width=\columnwidth]{tex/img/likert_ranking_uisx.png}
\caption{The proportion of bootstrapped samples (n=1000) of conversations (100 per bot) for which the bot rankings are the same. Bars denote ranking agreement for between-group $Stu$-$Sur$. Lines denote ranking agreement for within-group $Stu$ and $Sur$.}
\label{fig:likert_ranking}
\end{figure}

==> tex/fig/metrics.tex <==

%% Likert Dialogue

\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{tex/img/interactive_likert_dialogue.pdf}
\caption{Average Likert ratings for the 4 bots based on the interactive evaluations. Error bars denote bootstrapped 95\% confidence intervals for the average rating.}
\label{fig:interactive_likert_dialogue}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{tex/img/external_likert_dialogue.pdf}
\caption{Average Likert ratings for the 4 bots based on the external evaluations. Error bars denote bootstrapped 95\% confidence intervals for the average rating.}
\label{fig:external_likert_dialogue}
\end{figure*}

%% Comparative

\begin{figure*}[htb]
\centering
\includegraphics[width=0.75\textwidth]{tex/img/interactive_comparative.pdf}
\caption{Win/Tie/Lose proportions for the 4 bots based on the interactive evaluations. Error bars denote bootstrapped 95\% confidence intervals for the win proportion.}
\label{fig:interactive_comparative}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=0.75\textwidth]{tex/img/external_comparative.pdf}
\caption{Win/Tie/Lose proportions for the 4 bots based on the external evaluations. Error bars denote bootstrapped 95\% confidence intervals for the win proportion.}
\label{fig:external_comparative}
\end{figure*}


==> tex/fig/metrics_by_bot.tex <==
%% Likert Dialogue

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{tex/img/BART-FiD-RAG_likert_dialogue.pdf}
\caption{Average Likert ratings for BART-FiD-RAG from interactive evaluations (red) and external evaluations (gray). Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (paired t-test).}
\label{fig:BART-FiD-RAG_likert_dialogue}
\end{figure*}

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{tex/img/Blender-Decode_likert_dialogue.pdf}
\caption{Average Likert ratings for Blender-Decode from interactive evaluations (red) and external evaluations (gray). Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (paired t-test).}
\label{fig:Blender-Decode_likert_dialogue}
\end{figure*}

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{tex/img/Blender2_likert_dialogue.pdf}
\caption{Average Likert ratings for Blender2 from interactive evaluations (red) and external evaluations (gray). Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (paired t-test).}
\label{fig:Blender2_likert_dialogue}
\end{figure*}

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{tex/img/emora_likert_dialogue.pdf}
\caption{Average Likert ratings for Emora from interactive evaluations (red) and external evaluations (gray). Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (paired t-test).}
\label{fig:emora_likert_dialogue}
\end{figure*}

%% Comparative

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{tex/img/BART-FiD-RAG_comparative.pdf}
\caption{Comparative results for BART-FiD-RAG vs all other bots from interactive evaluations (red) and external evaluations (gray). Win/tie/loss rates are shown from top-to-bottom. Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (z-test of proportions).}
\label{fig:BART_FiD_RAG_comparative}
\end{figure*}

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{tex/img/Blender-Decode_comparative.pdf}
\caption{Comparative results for Blender-Decode vs all other bots from interactive evaluations (red) and external evaluations (gray). Win/tie/loss rates are shown from top-to-bottom. Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (z-test of proportions).}
\label{fig:Blender_Decode_comparative}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{tex/img/Blender2_comparative.pdf}
\caption{Comparative results for Blender2 vs all other bots from interactive evaluations (red) and external evaluations (gray). Win/tie/loss rates are shown from top-to-bottom. Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (z-test of proportions).}
\label{fig:Blender2_comparative}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{tex/img/Emora_comparative.pdf}
\caption{Comparative results for Emora vs all other bots from interactive evaluations (red) and external evaluations (gray). Win/tie/loss rates are shown from top-to-bottom. Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (z-test of proportions).}
\label{fig:Emora_comparative}
\end{figure*}

==> tex/fig/predictive_validity.tex <==

% \begin{figure*}[htb]
% \centering
% \includegraphics[width=\textwidth]{tex/img/pred_valid_int.pdf}
% \caption{Extent to which each turn-level evaluation metric can explain variance in interactive conversation quality by fitting a univariate regression model ($R^2$ for predicting $Qua_d$ using linear regression, McFadden’s Pseudo-$R^2$ for predicting $Qua_c$ using logistic regression).}
% \label{fig:interactive_predictive_validity}
% \end{figure*}

% \begin{figure*}[htb]
% \centering
% \includegraphics[width=\textwidth]{tex/img/pred_valid_ext.pdf}
% \caption{Extent to which each turn-level evaluation metric can explain variance in external conversation quality by fitting a univariate regression model ($R^2$ for predicting $Qua_d$ using linear regression, McFadden’s Pseudo-$R^2$ for predicting $Qua_c$ using logistic regression).}
% \label{fig:external_predictive_validity}
% \end{figure*}


\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{tex/img/pred_valid_likert.png}
\caption{Extent to which each turn-level evaluation metric can explain variance in Likert Quality for interactive and external evaluations by fitting univariate regression models ($R^2$ for predicting $Qua_d$ using linear regression).}
\label{fig:predictive_validity_likert}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{tex/img/pred_valid_comp.png}
\caption{Extent to which each turn-level evaluation metric can explain variance in Comparative Quality for interactive and external evaluations by fitting univariate regression models (McFadden’s Pseudo-$R^2$ for predicting $Qua_c$ using logistic regression).}
\label{fig:predictive_validity_comparative}
\end{figure*}

% \begin{figure*}[htb]
% \centering
% \includegraphics[width=\textwidth]{tex/img/pred_valid_comparative.pdf}
% \caption{Extent to which each turn-level evaluation metric can explain variance in Comparative Quality for interactive and external evaluations by fitting a univariate regression model ($R^2$ for predicting $Qua_d$ using linear regression, McFadden’s Pseudo-$R^2$ for predicting $Qua_c$ using logistic regression).}
% \label{fig:external_predictive_validity}
% \end{figure*}

==> tex/fig/sensitivity_cost_analysis.tex <==

\begin{figure*}[htb]
\centering
\includegraphics[width=0.75\textwidth]{tex/img/sensitivity_cost_analysis.pdf}
\caption{The rate of significant differences for each bot-pair as a function of the quantity of evaluated dialogues, according to both interactive and external evaluations. Rates were determined as the number of samples that produced significant results (t-test) out of 1000 random samples at each dialogue quantity.}
\label{fig:sensitivity_cost_analysis}
\end{figure*}

==> tex/limitations.tex <==
\section{Limitations}

One limitation of this work is that two of the groups ($Stu_x$ and $Dev_x$) did not provide complete evaluations for the 400 dialogues in the utilized dataset for both Likert and Pairwise evaluations  (refer to Appendix \ref{app:collection_limitations}), and were especially lacking in the size of the doubly annotated conversations within-group for the IAA analysis. Although the findings presented in this work indicate certain effects of the explored evaluator groups on evaluation consistency, further work with greater statistical power is needed to gain a more complete picture of the impact of different evaluator groups on dialogue evaluation results.

In addition, exploring differences resulting from groups that vary on other characteristics is also important to round out the findings of this work. For instance, one popular and convenient evaluator group for dialogue work is crowdsourcing, such as through Amazon Mechanical Turk, which was not explored here. Similarly, only 4 bots were explored in this work, which provides a limited view of the range of dialogue models produced in the field.

It should also be mentioned that there is a small amount of work on optimizing the within-group agreement for Pairwise evaluations of dialogue models. For instance, \citet{li:20} present a small-scale study of the impact of different phrasings for dialogue metrics, noticing that it is possible to increase IAA through surface-level modifications even though the underlying semantic content of the evaluation questions are not changed. The evaluation setup that we follow from \citet{finch:23} does not perform any such optimization. Thus, it is possible that even the cross-evaluator-group agreements could be improved beyond that observed in this work through comprehensive investigation of such optimization, although that was beyond the scope of this work.

==> tex/methods.tex <==

\section{Methods}

\input{tex/agreement}

\input{tex/effect_size}

==> tex/multifig/all_comparative.tex <==

\begin{figure*}[htb]
\centering
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/BART-FiD-RAG_comparative.pdf}
    \caption{BART-FiD-RAG}
    \label{fig:BART_FiD_RAG_comparative}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/Blender-Decode_comparative.pdf}
    \caption{Blender-Decode}
    \label{fig:Blender_Decode_comparative}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/Blender2_comparative.pdf}
    \caption{Blender2}
    \label{fig:Blender2_comparative}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/Emora_comparative.pdf}
    \caption{Emora}
    \label{fig:Emora_comparative}
\end{subfigure}
\caption{Win rates for each bot vs all other bots from interactive evaluations (red) and external evaluations (gray). Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (z-test of proportions, \textit{p} < 0.05).}
\label{fig:all_comparative}
\end{figure*}



==> tex/multifig/all_likert.tex <==

\begin{figure*}[htb]
\centering
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/BART-FiD-RAG_likert_dialogue.pdf}
    \caption{BART-FiD-RAG}
    \label{fig:BART-FiD-RAG_likert_dialogue}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/Blender-Decode_likert_dialogue.pdf}
    \caption{Blender-Decode}
    \label{fig:Blender-Decode_likert_dialogue}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/Blender2_likert_dialogue.pdf}
    \caption{Blender2}
    \label{fig:Blender2_likert_dialogue}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/emora_likert_dialogue.pdf}
    \caption{Emora}
    \label{fig:emora_likert_dialogue}
\end{subfigure}
\caption{Average Likert ratings for each bot from interactive evaluations (red) and external evaluations (gray). Error bars denote bootstrapped 95\% confidence intervals. Boxed labels indicate statistically significant differences between the two rater groups (paired t-test, \textit{p} < 0.05).}
\label{fig:all_likert}
\end{figure*}

==> tex/multifig/ranking.tex <==

\begin{figure}[htb]
\centering
\begin{subfigure}{\columnwidth}
    \includegraphics[width=\textwidth]{tex/img/likert_ranking_uisx.png}
    \caption{Likert}
    \label{fig:likert_ranking}
\end{subfigure}
\begin{subfigure}{\columnwidth}
    \includegraphics[width=\textwidth]{tex/img/comparative_ranking_uisx.png}
    \caption{Pairwise}
    \label{fig:comparative_ranking}
\end{subfigure}
\caption{The proportion of bootstrapped samples (n=10,000) of conversations (100 per bot) for which the bot rankings are the same. Bars denote ranking agreement for between-group $Stu$-$Sur$. Lines denote ranking agreement for within-group $Stu$ and $Sur$.}
\label{fig:ranking}
\end{figure}

==> tex/multifig/sensitivity.tex <==

\begin{figure*}[htb]
\centering
\begin{subfigure}{0.75\textwidth}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|llllll|l||l|llllll}
     & \multicolumn{3}{c}{EM} & \multicolumn{2}{c}{B2} & BD & \multirow{2}{*}{\#} & \multirow{2}{*}{\#} & BD & \multicolumn{2}{c}{B2} & \multicolumn{3}{c}{EM} \\
     & B2 & BD & BFR & BD & BFR & BFR &  &  & BFR & BFR & BD & BFR & BD & B2 \\ \hline
    Con$_d$ &&&&&&& 0 & \red 4 & \redcheck & \redcheck & & \redcheck && \redcheck \\
    Emo$_d$ &\blackcheck&&&\blackcheck&\blackcheck&& 3 & 3 &&\blackcheck&\blackcheck&&&\blackcheck\\
    Eng$_d$ & \redcheck &&\blackcheck& \redcheck &\blackcheck&\blackcheck& \red 5 & 3 &\blackcheck&\blackcheck&&\blackcheck&&\\
    Gra$_d$ &&\blackcheck&&\blackcheck&\blackcheck& \redcheck & 4 & 4 &&\blackcheck&\blackcheck&& \blackcheck & \redcheck \\
    Inf$_d$ &&\blackcheck&\blackcheck&&&& 2 & \red 3 &&& \redcheck &\blackcheck&\blackcheck&\\
    Pro$_d$ &&&\blackcheck&&\blackcheck&\blackcheck& 3 & 3 &\blackcheck&\blackcheck&&\blackcheck&&\\
    Qua$_d$ & \redcheck &&\blackcheck&\blackcheck&\blackcheck&\blackcheck& \red 5 & 4 &\blackcheck&\blackcheck&\blackcheck&\blackcheck&&\\
    Rel$_d$ &\blackcheck&&&\blackcheck&\blackcheck&& 3 & 3 &&\blackcheck&\blackcheck&&&\blackcheck\\
    \hline
    Con$_c$ &&&& \redcheck && \redcheck & \red 2 & 1 &&&&&& \redcheck \\
    Emo$_c$ &&&&&&& 0 & 0 &&&&&&\\
    Eng$_c$ &&& \redcheck && \redcheck &\blackcheck& \red 3 & 1 &\blackcheck&&&&&\\
    Gra$_c$ &&&& \redcheck &&& \red 1 & 0 &&&&&&\\
    Inf$_c$ &&& \redcheck &&\blackcheck&& 2 & 2 &&\blackcheck&&& \redcheck &\\
    Pro$_c$ & \redcheck && \redcheck && \redcheck &\blackcheck& \red 4 & 1 &\blackcheck&&&&&\\
    Qua$_c$ &&&& \redcheck && \redcheck & \red 2 & 0 &&&&&&\\
    Rel$_c$ &&&& \redcheck && \redcheck & \red 2 & 0 &&&&&&
    \end{tabular}%
    }
    \caption{Significant differences detected between the 6 bot-pairs with 100 dialogues per bot for both interactive evaluations (left) and external evaluations (right). Red denotes higher sensitivity.}
    \label{tab:sensitivity}  
\end{subfigure}
\begin{subfigure}{0.75\textwidth}
    \includegraphics[width=\textwidth]{tex/img/sensitivity_cost_analysis.pdf}
    \caption{The rate of significant differences in Likert Quality for each bot-pair as a function of the quantity of evaluated dialogues, according to both interactive and external evaluations. Rates were determined as the number of samples that produced significant results (t-test) out of 1000 random samples at each dialogue quantity.}
    \label{fig:sensitivity_cost_analysis}  
\end{subfigure}
\caption{Sensitivity results for bot-pair differences (\textit{p} < 0.05)}
\label{fig:sensitivity_results}
\end{figure*}

==> tex/notes.tex <==
- make y-scales the same for effect size diff
- update subscript for likert
- psychology: likert rating, sampling group, participant sampling, preferences, cognitive task
- make note of difficulty of getting student evaluators vs interactive student communicators


==> tex/old/eval_metrics_table.tex <==

\begin{table}[ht]
\centering\resizebox{\columnwidth}{!}{
  \begin{tabular}{rp{2cm}||p{6cm}}
  & \bf Dimension & \bf Definition\\
  \hline\hline
  \tt \textbf{Gra}: \tt & \tt Grammaticality & Responses are free of grammatical and semantic errors \\
  \tt \textbf{Rel}: & \tt Relevance & Responses are on-topic with the immediate dialogue history \\
  \tt \textbf{Inf}: & \tt Informativeness & Responses produce unique and non-generic information that is specific to the dialogue context \\
  \tt \textbf{Emo}: & \tt Emotional Understanding & Responses indicate an understanding of the user's current emotional state and provide an appropriate emotional reaction based on the current dialogue context \\
  \tt \textbf{Eng}: & \tt Engagingness & Responses are engaging to user and fulfill the particular conversational goals implied by the user \\
  \tt \textbf{Con}: & \tt Consistency & Responses do not produce information that contradicts other information known about the system \\
  \tt \textbf{Pro}: & \tt Proactivity & Responses actively and appropriately move the conversation along different topics \\
  \tt \textbf{Qua}: & \tt Quality & The overall quality of and satisfaction with the dialogue \\
  \end{tabular}}
  \caption{8 dialogue evaluation metrics; table adapted from \citet{finch_towards:20}}
  \label{tab:dims}
\end{table}

==> tex/old/ranking.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Macro-level Reproducibility}

As discussed in \sref{sec:related_work}, the aggregate results of evaluations are more appropriate when assessing the utility of evaluation procedures for dialogue evaluations. Since a low agreement on conversation-level decisions do not necessarily lead to a low agreement on aggregate system-level outcomes, it is important to measure the reproducibility of aggregate outcomes as well when assessing an evaluation method. To this end, a bot ranking metric (\sref{sec:bot_ranking}) and a bot-pair sensitivity metric (\sref{sec:botpair_sensitivity}) are utilized.

\subsection{Bot Ranking}
\label{sec:bot_ranking}

The desired outcome of any dialogue evaluation method is an understanding of which dialogue models perform better than others. One way to represent this is as a relative rank-ordering of the bots under evaluation. For Likert evaluations, this rank-ordering can be achieved averaging the Likert ratings given to the conversations of each bot. For Pairwise evaluations, this rank-ordering can be achieved using the proportion of wins each bot receives against all other bots. To measure the reproducibility of the bot rankings, bootstrapping is used to simulate random draws of evaluations from each annotator group. The proportion of bootstrapped samples for which the rankings agree is then the reproducibility of the rankings.

% \input{tex/fig/likert_ranking}
% \input{tex/fig/comparative_ranking}

\input{tex/multifig/ranking}

Figures \ref{fig:likert_ranking} and \ref{fig:comparative_ranking} show the ranking agreements for between-group $Stu$-$Sur$ evaluations and for within-group $Sur$ evaluations and within-group $Stu$ evaluations for Likert and Pairwise evaluations, respectively. It is clear that the $Stu$ and $Sur$ groups are more in agreement on the Likert rankings of the bots, than on the Pairwise rankings, with the ranking agreements between $Stu$ and $Sur$ approaching the within-group ranking agreements for many of the evaluation dimensions. Even though the within-group ranking agreements for Pairwise evaluations can be high, there is low between-group ranking agreement for all of the dimensions which overwhelming suggests that these pairwise evaluations are not reproducible across different groups of annotators. 


% \input{tex/tab/ranking_agreements}


==> tex/old/sensitivity.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Bot-pair Sensitivity}
\label{sec:botpair_sensitivity}

It is also important for dialogue evaluation methods to be sensitive to the differences between different dialogue models. If an evaluation is unable to reliably detect differences between bots, then it is not an informative methodology. To assess the strength and reproducibility of an evaluation's sensitivity to bot-pair differences, statistical testing procedures are applied to the evaluations produced by each group and the sensitivity rates are compared. The number of bot-pairs whose differences are statistically significant are shown in Table \ref{tab:sensitivity_combined} for each dimension for Likert and Pairwise evaluations. 

% \input{tex/tab/sensitivity_likert}

% \input{tex/tab/sensitivity_comparative}

\input{tex/tab/sensitivity_combined}

For Likert, the evaluations from both $Stu$ and $Sur$ achieve similar sensitivities for most dimensions, with the exception of $Con_d$ and $Eng_d$. On the other hand, there is greater variation in the sensitivity of Pairwise evaluations between $Stu$ and $Sur$ with $Eng_c$, $Gra_c$, $Pro_c$, $Qua_c$, and $Rel_c$ resulting a difference of 2 or more significant bot-pairs.

==> tex/results.tex <==
\input{tex/agreement}

\input{tex/effect_size}

==> tex/resultsdiscussion.tex <==

\section{Results and Discussion}

\subsection{Level of Analysis: Dialogue vs. Bot}



\subsection{Chatbot Developers as Evaluators}

\begin{figure*}
\centering
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/likert_agreement_bar_experts.png}
    \caption{Likert}
    \label{fig:likert_agreement_expert}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/comparative_agreement_bar_experts.png}
    \caption{Pairwise}
    \label{fig:comparative_agreement_expert}
\end{subfigure}
\caption{Comparison of IAA achieved between experts and novices vs. IAA achieved within novices themselves. Error bars denote bootstrapped 95\% confidence intervals for the average rating.}
\label{fig:agreement_expert}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/effect_size_difference_likert_experts.png}
    \caption{Likert}
    \label{fig:likert_ef_expert}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/effect_size_difference_comparative_experts.png}
    \caption{Pairwise}
    \label{fig:comparative_ef_expert}
\end{subfigure}
\caption{Comparison of differences in effect size between experts and novices vs. within novices themselves. Error bars denote bootstrapped 95\% confidence intervals for the average rating.}
\label{fig:ef_expert}
\end{figure*}

The results of this study suggest that there is a substantial difference between the evaluations conducted by chatbot developers and those conducted by novice evaluators. Each of the interactive students, external students, and Surgers utilized in this work can be considered novice evaluators since they are not specialized in the development of chatbots. It is clear from Figures \ref{fig:ef_likert} and \ref{fig:ef_comparative} that the largest changes in effect size are primarily resulting from the comparison between some novice group to the developer group. This is the case for $Gra_d$, $Inf_d$, $Pro_d$, and $Eng_d$ for Likert as well as for $Con_c$, $Emo_c$, $Eng_d$, $Gra_d$, $Inf_c$, $Qua_c$, and $Rel_d$ for Pairwise. The other comparisons for these dimensions produce much reduced differences between the compared groups; thus suggesting that the developer group is a major source of such extreme differences.

\subsection{Novice Evaluators}

\begin{figure*}
\centering
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/likert_agreement_bar_novice.png}
    \caption{Likert}
    \label{fig:likert_agreement_novice}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/comparative_agreement_bar_novice.png}
    \caption{Pairwise}
    \label{fig:comparative_agreement_novice}
\end{subfigure}
\caption{Comparison of IAA achieved between each of the novice groups. Error bars denote bootstrapped 95\% confidence intervals for the average rating.}
\label{fig:agreement_novice}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/effect_size_difference_likert_novice.png}
    \caption{Likert}
    \label{fig:likert_ef_novice}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{tex/img/effect_size_difference_comparative_novice.png}
    \caption{Pairwise}
    \label{fig:comparative_ef_novice}
\end{subfigure}
\caption{Comparison of differences in effect size between novice groups. Error bars denote bootstrapped 95\% confidence intervals for the average rating.}
\label{fig:ef_novice}
\end{figure*}

For most Likert dimensions, both the interactive and external student groups are able to achieve reasonable agreement with each other as well as the Surgers, with changes in effect size usually at 0.2 or lower. The same holds true for most Pairwise dimensions, although the observed changes in effect size are usually slightly higher at 0.3 or lower.

For most Likert and Pairwise dimensions,the Surgers are able to achieve reasonable agreement with all of the student groups, with changes in effect size usually at 0.2 or lower. One interesting observation is that the Surgers achieve the most similar evaluations to all of the other groups for the $Qua_d$ dimension. It could be the case that Surgers are effective at estimating the rating that most people would agree with, since they are trained and incentivized to provide high agreement with others in their annotations for NLP tasks in general.

\subsection{Point-of-View Robustness}
Most dimension of Likert evaluations seem to be robust to a change in the evaluator point-of-view. The difference in effect size between external students and interactive students is quite low, at or below 0.2 for all dimensions except for $Emo_d$. This provides some evidence that the level of involvement that the evaluator has in the dialogue that they are evaluating (e.g. whether they are the interactor or an external third-party to the dialogue) does not change the evaluations that they provide. In terms of the outlier $Emo_d$, it can be seen that the external student group experiences the highest disagreement with \textbf{all} of the other groups; thus, it seems that the external students have a different definition of utterance emotional appropriateness or a more noisy evaluation output as compared to the other groups, not just due to a change in evaluator point-of-view.

A similar phenomenon occurs for Pairwise evaluations, since it can be seen that the change from external students to interactive students results in some of the lowest changes in effect size relative to other cross-group comparisons. This seems to be true for all Pairwise dimensions.


\subsection{Dimension Robustness}

Interestingly, substantial cross-evaluator-group disagreement is not observed for the $Qua_d$, $Rel_d$ and $Con_d$ dimensions; EAch of these dimensions seems to be quite robust to changes in evaluator group, with the lowest differences in effect sizes and IAA reductions observed across all groups. This is encouraging for $Qua_d$ in particular, since it is often the metric used in dialogue model works to provide a holistic evaluation of the performance of a bot.

\subsubsection{Evaluator Group Advantages}

For $Con_d$ specifically, though, there is some weak evidence that external students and Surgers produce the most similar evaluations to one another, with the change in effect size effectively improving by 50\% compared to the other group comparisons. It could be the case that the external nature of these groups is the determining characteristic for making decisions on certain dimensions. Intuitively, $Con$ is one of the least subjective dialogue characteristics as it relies less on personal impressions and more on explainable observations, such as context contradictions, and having a less personal interface into the dialogue through external evaluations could strongly govern the evaluation decisions. 

\subsection{Method Robustness}
Overall, the Likert evaluations seem to be more robust to changes in evaluator group than Pairwise evaluations, producing less dramatic changes in effect size and interannotator agreement. This is especially true when considering the non-developer group comparisons, which are the most practical groups to select from for dialogue model evaluations. The changes in effect sizes for such group comparisons are consistently smaller for Likert than for Pairwise, which is desirable.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The results of the IAA and effect size analyses reveal that it is possible for a change in evaluator group to produce a substantial discrepancy in chatbot evaluation, depending on which evaluation method and evaluation dimension are being used. Overall, it does seem to be that Likert evaluations are more robust to changes in evaluator group than Pairwise evaluations, both on the dialogue- and bot-level. Changing the evaluator group results in only a slight reduction in agreement on the ratings of dialogues for most Likert dimensions compared to the agreement observed between evaluators of the same group.  Similarly, for bot-level analysis, it can be said that changing evaluator group in Likert evaluations seems to have a low effect size in itself because the effect sizes of bot-pairs between different groups only differ by 0.2 or less for most dimensions, whereas for Pairwise comparisons the effect size of changing evaluator group is at least a moderate effect with a change in effect size of 0.3 or more for most dimensions.

% Notably, Likert evaluations of the $Qua_d$ dimension seem to be quite robust to changes in evaluator group, with one of the lowest differences in effect sizes and IAA reductions observed. This is encouraging as $Qua_d$ is often the metric used in dialogue model works to provide a holistic evaluation of the performance of a bot. A similar robustness is also observed for $Rel_d$, $Pro_d$, and $Emo_d$.

% On the other hand, there exist some dimensions that are more impacted by changes in evaluator group for Likert. This is most obvious for $Con_d$ since it experiences one of the highest drops in IAA agreement and one of the largest differences in effect size between the two evaluator groups. Intuitively, $Con$ is one of the least subjective dialogue characteristics as it relies less on personal impressions and more on explainable observations, such as context contradictions. A similar effect is observed for the $Inf_d$ dimension, which also shares a certain underpinning of objectivity like $Con_d$. In practice, it may be the case that such objective dimensions like $Con_d$ and $Inf_d$ are better captured by experienced external evaluators than inexperienced or interactive evaluators.

% It is also observed that $Gra_d$ has a near-zero IAA between the two evaluator groups and one of the highest changes in effect size between groups. However, unlike $Con_d$ and $Inf_d$, it is not the case that the $Sur$ group achieves a much higher IAA either; instead, $Gra_d$ has the lowest IAA for the $Sur$ group out of all of the Likert dimensions. It does not seem to be the case that this cross-group disagreement is likely to be explained by the $Sur$ group achieving a better evaluation than the $Stu$. Instead, the case of $Gra_d$ seems to be genuine disagreement on the Likert ratings; the overall distribution of Likert ratings for $Gra_d$ suggest that the $Stu$ group provides more extreme ratings for several of the bots than the $Sur$ group, thus leading to low agreement and a higher change in effect size between bot-pairs (see Appendix \sref{sec:likert_outcomes}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Taken alone, the within-group IAA agreements for $Sur$ in Figure \ref{fig:agreements} would suggest that Pairwise evaluations are able to improve upon the replicability of dialogue evaluations as compared to Likert, as the IAA agreements are better for several dimensions and approximately the same for the rest. However, this limited scope fails to assess the more practical utility of dialogue evaluation in which multiple groups of evaluators will be used to evaluate dialogue models over time. In this case, it is more representative to look at between-group agreements as a measure of the consistency and replicability of a particular evaluation method. The between-group IAA presents a different story than the within-group IAA, suggesting that Likert evaluation is able to achieve higher replicability than Pairwise as the between-group IAA's are higher.

% This finding is further corroborated by replicability analyses that target the aggregate outcome level of dialogue evaluation. The effect size analysis shows that there is little change in observed bot-pair differences between both evaluator groups for Likert evaluation, but this is not the case for Pairwise. Compared to the IAA analysis, the differences observed for these aggregate analyses is often of a more observable magnitude as well.

% Although Likert evaluations do result in many similar results from the different evaluator groups, there are a few key differences that may lend insight into the different strengths of types of evaluators for dialogue evaluation.

% From Figure \ref{fig:ef_diff_likert}, it is clear that the most disagreement in effect size occurs for $Con$.  Furthermore, the within-group IAA of $Sur$ for $Con$ is one of the highest relative to the other dimensions, and it also shows one of the largest drops in IAA when looking at $Stu$-vs-$Sur$ agreements as shown in Figure \ref{fig:agreements}. These results suggest that the $Sur$ group is able to more reliably evaluate $Con$ as compared to the $Stu$ group. Out of the dialogue dimensions, $Con$ is one of the least subjective dialogue characteristics as it relies less on personal impressions and more on explainable observations, such as context contradictions. To this end, the annotation experience of $Sur$ annotators coupled with the separation between the external $Sur$ evaluators and the dialogues they are evaluating may prove to be beneficial for these more objective dimensions. In practice, it may be the case that $Con_d$ is better captured by experienced external evaluators than inexperienced or interactive evaluators. 



==> tex/tab/annotator_stats.tex <==

\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l||c|ccc}
 % & \textbf{} & \multicolumn{3}{c}{\textbf{Units}} \\
 & \textbf{\#} & \textbf{Min} & \textbf{Med} & \textbf{Max} \\
 \hline \hline
\texttt{Ui} & 46 & 3 & 9 & 42 \\
\hspace*{0.5cm} \textit{Likert} & 46 & 2 & 6 & 28 \\
\hspace*{0.5cm} \textit{Comparative} & 46 & 1 & 3 & 14 \\
\hline
\texttt{Sx} & 32 & 1 & 14 & 103 \\
\hspace*{0.5cm} \textit{Likert} & 26 & 1 & 11 & 75 \\
\hspace*{0.5cm} \textit{Comparative} & 20 & 1 & 8 & 39
\end{tabular}%
}
\caption{Annotator statistics for the interactive and external annotator groups. \textbf{\#}: number of unique annotators. \textbf{Min/Med/Max}: minimum/median/maximum number of evaluation units completed by a single annotator.}
\label{tab:annotator_stats}
\end{table}

==> tex/tab/convo_agreements.tex <==
\begin{table}[htbp]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|llllllll}
 & \bf Con & \bf Emo & \bf Eng & \bf Gra & \bf Inf & \bf Pro & \bf Qua & \bf Rel \\
 \hline \hline
\bf \texttt{Ui / Sx} & 0.20 & 0.24 & 0.24 & 0.05 & 0.12 & 0.21 & 0.23 & 0.28 \\
\hline
\bf \texttt{Sx / Sx} & 0.36 & 0.26 & 0.26 & 0.13 & 0.41 & 0.24 & 0.29 & 0.30 \\
\hline \hline
\bf \texttt{Ui / Sx} & 0.01 & 0.13 & 0.10 & 0.12 & 0.06 & 0.13 & 0.16 & 0.11 \\
\hline
\bf \texttt{Sx / Sx} & 0.51 & 0.20 & 0.10 & 0.22 & 0.19 & 0.25 & 0.47 & 0.44
\end{tabular}%
}
\caption{Krippendorf's alpha for conversation evaluations between various annotator groups.}
\label{tab:convo_agreements}
\end{table}

==> tex/tab/ranking_agreements.tex <==

\begin{table}[htpb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l||llllllll}
 & \bf Rel & \bf Qua & \bf Gra & \bf Con & \bf Emo & \bf Eng & \bf Inf & \bf Pro \\
 \hline \hline
\bf \texttt{Ui / Sx} & 0.28 & 0.47 & 0.81 & 0.19 & 0.46 & 0.24 & 0.15 & 0.32 \\
\hline
\bf \texttt{Ui / Ui} & 0.29 & 0.46 & 0.78 & 0.15 & 0.33 & 0.53 & 0.19 & 0.36 \\
\bf \texttt{Sx / Sx} & 0.26 & 0.62 & 0.84 & 0.67 & 0.40 & 0.43 & 0.39 & 0.25 \\
\hline \hline
\bf \texttt{Ui / Sx} & 0.02 & 0.01 & 0.04 & 0.01 & 0.13 & 0.03 & 0.03 & 0.07 \\
\hline
\bf \texttt{Ui / Ui} & 0.40 & 0.66 & 0.29 & 0.37 & 0.28 & 0.32 & 0.49 & 0.37 \\
\bf \texttt{Sx / Sx} & 0.17 & 0.16 & 0.10 & 0.65 & 0.18 & 0.45 & 0.83 & 0.70
\end{tabular}%
}
\caption{Percentage of bootstrapped samples in which the two annotator groups agreed on the ranked bot performance.}
\label{tab:ranking}
\end{table}

==> tex/tab/sensitivity.tex <==

\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|llllll|l||l|llllll}
 & \multicolumn{3}{c}{EM} & \multicolumn{2}{c}{B2} & BD & \multirow{2}{*}{total} & \multirow{2}{*}{total} & BD & \multicolumn{2}{c}{B2} & \multicolumn{3}{c}{EM} \\
 & B2 & BD & BFR & BD & BFR & BFR &  &  & BFR & BFR & BD & BFR & BD & B2 \\ \hline
Con$_d$ &&&&&&& 0 & \red 4 & \redcheck & \redcheck & & \redcheck && \redcheck \\
Emo$_d$ &\blackcheck&&&\blackcheck&\blackcheck&& 3 & 3 &&\blackcheck&\blackcheck&&&\blackcheck\\
Eng$_d$ & \redcheck &&\blackcheck& \redcheck &\blackcheck&\blackcheck& \red 5 & 3 &\blackcheck&\blackcheck&&\blackcheck&&\\
Gra$_d$ &&\blackcheck&&\blackcheck&\blackcheck& \redcheck & 4 & 4 &&\blackcheck&\blackcheck&& \blackcheck & \redcheck \\
Inf$_d$ &&\blackcheck&\blackcheck&&&& 2 & \red 3 &&& \redcheck &\blackcheck&\blackcheck&\\
Pro$_d$ &&&\blackcheck&&\blackcheck&\blackcheck& 3 & 3 &\blackcheck&\blackcheck&&\blackcheck&&\\
Qua$_d$ & \redcheck &&\blackcheck&\blackcheck&\blackcheck&\blackcheck& \red 5 & 4 &\blackcheck&\blackcheck&\blackcheck&\blackcheck&&\\
Rel$_d$ &\blackcheck&&&\blackcheck&\blackcheck&& 3 & 3 &&\blackcheck&\blackcheck&&&\blackcheck\\
\hline
Con$_c$ &&&& \redcheck && \redcheck & \red 2 & 1 &&&&&& \redcheck \\
Emo$_c$ &&&&&&& 0 & 0 &&&&&&\\
Eng$_c$ &&& \redcheck && \redcheck &\blackcheck& \red 3 & 1 &\blackcheck&&&&&\\
Gra$_c$ &&&& \redcheck &&& \red 1 & 0 &&&&&&\\
Inf$_c$ &&& \redcheck &&\blackcheck&& 2 & 2 &&\blackcheck&&& \redcheck &\\
Pro$_c$ & \redcheck && \redcheck && \redcheck &\blackcheck& \red 4 & 1 &\blackcheck&&&&&\\
Qua$_c$ &&&& \redcheck && \redcheck & \red 2 & 0 &&&&&&\\
Rel$_c$ &&&& \redcheck && \redcheck & \red 2 & 0 &&&&&&
\end{tabular}%
}
\caption{Significant differences detected between the 6 bot-pairs for each metric for both interactive evaluations (left) and external evaluations (right). Red denotes the detection of more differences.}
\label{tab:sensitivity}
\end{table}

==> tex/tab/sensitivity_brief.tex <==


\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|llllllll|llllllll}
& \rot{Con$_d$} & \rot{Emo$_d$} & \rot{Eng$_d$} & \rot{Gra$_d$} & \rot{Inf$_d$} & \rot{Pro$_d$} & \rot{Qua$_d$} & \rot{Rel$_d$} & \rot{Con$_c$} & \rot{Emo$_c$} & \rot{Eng$_c$} & \rot{Gra$_c$} & \rot{Inf$_c$} & \rot{Pro$_c$} & \rot{Qua$_c$} & \rot{Rel$_c$} \\
\hline
\bf Int & 0 & 3 & \bf 5 & 4 & 2 & 3 & \bf 5 & 3 & \bf 2 & 0 & \bf 3 & \bf 1 & 2 & \bf 4 & \bf 2 & \bf 2\\
\bf Ext & \bf 4 & 3 & 3 & 4 & \bf 3 & 3 & 4 & 3 & 1 & 0 & 1 & 0 & 2 & 1 & 0 & 0\\
\end{tabular}%
}
\caption{Significant differences (\textit{p} < 0.05) detected between the 6 bot-pairs for each metric for both interactive and external evaluations. \textbf{Int}: Interactive, \textbf{Ext}: External}
\label{tab:sensitivity_brief}
\end{table}




==> tex/tab/sensitivity_combined.tex <==


\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|llllllll||llllllll}
& \rot{Con$_d$} & \rot{Emo$_d$} & \rot{Eng$_d$} & \rot{Gra$_d$} & \rot{Inf$_d$} & \rot{Pro$_d$} & \rot{Qua$_d$} & \rot{Rel$_d$} 
& \rot{Con$_c$} & \rot{Emo$_c$} & \rot{Eng$_c$} & \rot{Gra$_c$} & \rot{Inf$_c$} & \rot{Pro$_c$} & \rot{Qua$_c$} & \rot{Rel$_c$} \\
\hline
\bf \texttt{Stu} & 0 & 3 & \bf 5 & 4 & 2 & 3 & \bf 5 & 3 & 
\bf 2 & 0 & \bf 3 & \bf 2 & 2 & \bf 3 & \bf 3 & \bf 3 \\
\bf \texttt{Sur} & \bf 4 & 3 & 3 & 4 & \bf 3 & 3 & 4 & 3 &
1 & 0 & 1 & 0 & 2 & 1 & 0 & 0\\
\end{tabular}%
}
\caption{Significant differences between the 6 bot-pairs for each metric. Likert: t-test, $n$=100, \textit{p} < 0.05. Pairwise: sign test, $n$=32, \textit{p} < 0.05.}
\label{tab:sensitivity_combined}
\end{table}


% \begin{table}[htb]
% \centering
% \resizebox{0.6\columnwidth}{!}{%
% \begin{tabular}{l|llllllll}
% & \rot{Con$_c$} & \rot{Emo$_c$} & \rot{Eng$_c$} & \rot{Gra$_c$} & \rot{Inf$_c$} & \rot{Pro$_c$} & \rot{Qua$_c$} & \rot{Rel$_c$} \\
% \hline
% \bf \texttt{Stu} 
% \bf \texttt{Sur} & \\
% \end{tabular}%
% }
% \caption{Significant differences (sign test, $n$=32, \textit{p} < 0.05) between the 6 bot-pairs for each Pairwise metric.}
% \label{tab:sensitivity_comparative}
% \end{table}

==> tex/tab/sensitivity_comparative.tex <==

\begin{table}[htb]
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{l|llllllll}
& \rot{Con$_c$} & \rot{Emo$_c$} & \rot{Eng$_c$} & \rot{Gra$_c$} & \rot{Inf$_c$} & \rot{Pro$_c$} & \rot{Qua$_c$} & \rot{Rel$_c$} \\
\hline
\bf \texttt{Stu} & \bf 2 & 0 & \bf 3 & \bf 2 & 2 & \bf 3 & \bf 3 & \bf 3\\
\bf \texttt{Sur} & 1 & 0 & 1 & 0 & 2 & 1 & 0 & 0\\
\end{tabular}%
}
\caption{Significant differences (sign test, $n$=32, \textit{p} < 0.05) between the 6 bot-pairs for each Pairwise metric.}
\label{tab:sensitivity_comparative}
\end{table}

==> tex/tab/sensitivity_likert.tex <==

\begin{table}[htb]
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{l|llllllll}
& \rot{Con$_d$} & \rot{Emo$_d$} & \rot{Eng$_d$} & \rot{Gra$_d$} & \rot{Inf$_d$} & \rot{Pro$_d$} & \rot{Qua$_d$} & \rot{Rel$_d$} \\
\hline
\bf \texttt{Stu} & 0 & 3 & \bf 5 & 4 & 2 & 3 & \bf 5 & 3 \\
\bf \texttt{Sur} & \bf 4 & 3 & 3 & 4 & \bf 3 & 3 & 4 & 3 \\
\end{tabular}%
}
\caption{Significant differences (t-test, $n$=100, \textit{p} < 0.05) between the 6 bot-pairs for each Likert metric.}
\label{tab:sensitivity_likert}
\end{table}

==> tex/tab/timing.tex <==

\begin{table}[htb]
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{l||lll}
 & \textbf{Med} & \textbf{Std} & \textbf{Cv} \\
\hline \hline
\textbf{Dialogue} & 8.08 & 5.62 & 0.70 \\
\hline
\textbf{Likert} & & & \\
\hspace*{0.5cm} \texttt{Ui} & 0.61 & 0.85 & 1.38 \\
\hspace*{0.5cm} \texttt{Sx} & 2.81 & 4.63 & 1.65 \\
\hline
\textbf{Comparative} & & & \\
\hspace*{0.5cm} \texttt{Ui} & 0.69 & 0.62 & 0.90 \\
\hspace*{0.5cm} \texttt{Sx} & 4.38 & 3.96 & 0.90
\end{tabular}%
}
\caption{Statistics on the completion times (in minutes). \textbf{Med/Std/Cv}: median/standard deviation/coefficient of variance of the completion times.}
\label{tab:timing}
\end{table}
